Learning to generate line drawings that convey geometry and semantics

This paper presents an unpaired method for creating line drawings from photographs. Current methods often rely on high quality paired datasets to generate line drawings. However, these datasets often have limitations due to the subjects of the drawings belonging to a specific domain, or in the amount of data collected. Although recent work in unsupervised image-to-image translation has shown much progress, the latest methods still struggle to generate compelling line drawings. We observe that line drawings are encodings of scene information and seek to convey 3D shape and semantic meaning. We build these observations into a set of objectives and train an image translation to map photographs into line drawings. We introduce a geometry loss which predicts depth information from the image features of a line drawing, and a semantic loss which matches the CLIP features of a line drawing with its corresponding photograph. Our approach outperforms state-of-the-art unpaired image translation and line drawing generation methods on creating line drawings from arbitrary photographs. For code and demo visit our webpage carolineec.github.io/informative_drawings

==> tables/semantics_img.tex <==
\begin{table}[ht!]
  \centering
  \resizebox{0.9\linewidth}{!}{
  \begin{tabular}{ccccc}
    \toprule
      & Contour Drawings & Anime & Total & Unknown  \\
\midrule
CycleGAN      &     $zzz$  &    $zzz$   &     $zzz$  &    $zzz$ \\ \hline
Ours          &     $zzz$  &    $zzz$   &     $zzz$  &    $zzz$ \\ \hline
Photograph    &     $-$    &    $-$     &     $zzz$  &    $zzz$ \\ 
    \bottomrule
  \end{tabular}
  }
  \caption{\caro{MSE error (lower is better)}} \label{table:semantics_img}
\end{table}

